A Distributed Transportation Simplex Applied to a Content Distribution Network Problem

A Content Distribution Network (CDN) can be defined as an overlay system that replicates copies of contents at multiple points of a network, close to the final users, with the objective of improving data access. CDN technology is widely used for the distribution of large-sized contents, like in video streaming. In this paper we address the problem of finding the best server for each customer request in CDNs, in order to minimize the overall cost. We consider the problem as a transportation problem and a distributed algorithm is proposed to solve it. The algorithm is composed of two independent phases: a distributed heuristic finds an initial solution that may be later improved by a distributed transportation simplex algorithm. It is compared with the sequential version of the transportation simplex and with an auction-based distributed algorithm. Computational experiments carried out on a set of instances adapted from the literature revealed that our distributed approach has a performance similar to its sequential counterpart, in spite of not requiring global information about the contents requests. Moreover, the results also showed that the new method outperforms the based-auction distributed algorithm.

==> distributed_algorithmf.tex <==
%%\section{Distributed Algorithm}
%
%%\include{sequential}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%-------------------------------------------------------------------
%
%%--------------------------------------------------------------------------------------------
%% SUBSECTION:   Sequential Transportation Simplex
%% SECTION:    Distributed Algorithm------------------------- 
%
%%--------------------------------------------------------------------------------------------
%% SUBSECTION:   Distributed Approach
%%-------------------------------------------------------------------------------------------- 
%\subsection{Distributed Approach}\label{subsec:distributed}
%
%In the  distributed algorithms described next, each server in $I$ is associated to a process, that executes the same local algorithm, which consists of sending messages, waiting for incoming messages and processing. Messages can be transmitted  independently and arrive  after an unpredictable but finite delay, without error and in sequence.  Processes have distinct identities that can be totally ordered. Initially, a server $i$ only knows the requests $(i,c)$, $c \in C_i$. On the other
%hand, it is assumed that a server knows which contents are present in each other server (possibly using a service similar to DNS) and the corresponding communication cost. The assumption is reasonable since content position change much less dynamically
%than request data.
%
%%--------------------------------------------------------------------------------------------
%% SUBSUBSECTION:  Initial Solution Algorithm DistPac
%%-------------------------------------------------------------------------------------------- 
%\subsubsection{Obtaining an Initial Solution}\label{subsubsec:initialdist}
%
%{\sl DistInit} is a distributed constructive heuristic, inspired by the Minimum Cost method, but not necessarily equivalent to it.
%In {\sl DistInit}, at first, each server tries to attend its local requests. If it is not capable of serving a local request, a message {\it Serve} is sent to the closest server that stores that content. Upon receiving this message, a server answers with an {\it ACK} or a {\it NACK} message depending on its bandwidth availability. When a server receives  a {\it NACK} or an {\it ACK} with partial attending, it sends another {\it Serve} message to the next closest server with the remaining required bandwidth.
%When all requests are attended, the algorithm finishes. In fact, there is a termination procedure not described here to detect this condition. See Figure \ref{fig:1} for  an example of a initial solution. Squares and circles represent servers and requests, respectively. The number inside the square is the server identification $i$, while the two numbers inside the circle of a request $j$ represent $(k(j),c(j))$. The edges indicate which servers attend each request.
%This solution can also be represented by a tree, as shown in Figure \ref{fig:2}(a).
%\begin{figure}[h]
%\centering
%\begin{center}
%\begin{tabular}{c}
%\includegraphics[scale=0.9]{figure/solinicial.pdf} \\
%\end{tabular}
%\end{center}
%\caption{Initial Solution}
%\label{fig:1}
%\end{figure}
%
%\begin{figure}[h]
%\centering
%
%\begin{tabular}{cc }
%\includegraphics[scale=0.8]{figure/arvore.pdf}&  
%\includegraphics[scale=0.8]{figure/arvore_com_custreduzido.pdf} \\
%{\bf {\footnotesize(a)}} &
%{\bf {\footnotesize(b)}} \\
%\end{tabular}
%
%\caption{(a) Solution Tree;  (b) Tree with Reduced Costs}
%\label{fig:2}
%\end{figure}
%
%
%%--------------------------------------------------------------------------------------------
%% SUBSUBSECTION:   Simplex Algorithm DistST
%%-----------------------------------------------------------------------------------------
%
%
%
%\subsubsection{Distributed Transportation Simplex}\label{subsubsec:simplexdist}
%
%The distributed transportation simplex ({\sl DistTS}) initiates in  the  server that has the smallest identification. It assigns  zero to its  dual variable $u_1$, calculates the dual variables $v$ corresponding to the requests supplied by it, and sends these values to the servers that hold those requests, through {\it Varv} messages. Upon receiving this message, each process calculates the dual variables of the other servers that have also contributed to attend a common request and sends these results through {\it Varu} messages.  This procedure is repeated, alternating the sending of {\it Varv} and {\it Varu} messages until all dual variables are calculated, and consequently the reduced costs, as shown in Figure \ref{fig:2}(b). Now, each server selects its most negative reduced cost edge and sends a message to the corresponding server, to introduce that non-basic variable in the solution. This procedure produces candidate cycles, as shown in Figure \ref{fig:3}(a).  
%Now,  messages are sent along the candidate cycles to select a basic variable to leave the solution. In the best case, this distributed algorithm can process all those cycles (i.e. make pivot steps) in parallel. However,  those candidate cycles may have intersections, which would cause inconsistencies if they are pivoted at the same time. So, when a conflict is detected, the cycle associated with the smallest reduced cost is chosen to continue, while the other is canceled. In the example of Figure \ref{fig:3}(a), the cycles have conflicts, and only one can be processed. If the smallest cycle
%is chosen, the new tree after the pivot is shown in Figure \ref{fig:3}(b). 
%For every pivot that is performed, it is
%also necessary to re-calculate the dual variables. However, instead of recalculating all of them, only the ones that belong to the new subtree are updated. The new dual variables are propagated  through {\it Varu} and {\it Varv} messages and all procedures described above are repeated until it is detected that there is no edge with negative reduced cost. 
%
%\begin{figure}[h]
%\centering
%
%\begin{tabular}{cc }
%\includegraphics[scale=0.7]{figure/ciclo.pdf}&  
%\includegraphics[scale=0.7]{figure/arvore_nova.pdf} \\
%{\bf {\footnotesize(a)}} &
%{\bf {\footnotesize(b)}} \\
%\end{tabular}
%
%\caption{(a) Cycles corresponding to edges with negative reduced cost;  (b) New tree after a pivot over the shorter cycle}
%\label{fig:3}
%\end{figure}
%
%% complexidade do algoritmo distribuido
\input{complex}

%\begin{tabular}{ll}
%\hline
%   Variables & Definitions\\
% \hline
%   $myId$ & $id$ associated with the server \\ 
%   $idMenor$ & servidor mais próximo (com menor custo de comunicação)\\
%   $servArtificial$ & servidor artificial\\
%   $banda$ & largura de banda disponível no servidor\\
%   $atendeu_{ic}$ & quantidade de banda alocada pelo servidor $meuId$ devido ao \\
%   & pedido do servidor $i$ pelo conteúdo $c$\\
%\hline
%   $req_r$ & requisição $r$ pertencente a $lReq$\\
%   $cont_r$ & identificação do conteúdo da requisição $r$ \\
%   $bandCont_r$ & tamanho da banda exigida pelo conteúdo da requisição $r$\\
%   $quantAlocada_r$ & quantidade de banda alocada para requisição $r$ \\ 
%   $atendimento_{ri}$ & quantidade de banda para requisição $r$ atendida pelo \\
%   & servidor $i$\\
%   $idReqArt$ & $id$ da requisição artificial atendida pelo servidor artificial\\   
%\hline
%   $S$ & Conjunto de Servidores\\
%   $lCont$ & Lista de todos os Conteúdos\\
%   $lReq$ & Lista de Requisições\\
%   $nReq$ & Número de Requisições \\
%   $lReqNalocadas$ & lista de requisições não alocadas do servidor\\
%   $lAcabou$ & lista de servidores que suspeitam que acabaram \\  
%\end{tabular}
%
%\begin{tabular}{ll} 
% \hline
%   Variables & Definitions\\
% \hline
%   $servInicial$ & $id$ do servidor que inicializa o segundo passo do simplex\\
%   $dualU$ & valor da variável dual $u$\\
%   $servPaiDU$ & servidor Pai da variável dual $u$ \\
%   $reqPaiDU$ & requisição Pai da variável dual $u$\\
%   $custo_{is}$ & distância entre o servidor $i$ e o servidor $s$\\  
%   $passo$ & número do passo do Simplex de Transporte\\
%   $caminhoServ$ & caminho na árvore de solução $T$ desde da raiz $sT$ até o servidor \\
%   &(cada posição corresponde a um servidor $\{s\}$ ou a uma $3-upla$ \\
%   & $<$servidor, requisição, $cont_{requisicao}>$ - $\{s,r,c\}$)\\
%   $caminhoServTam$ & tamanho do caminho na árvore de solução $T$ desde da raiz até o  \\
%   & servidor $sT$\\
%   $menorEscolhido$& servidor com menor $id$ de uma requisição alcançada pela construção\\
%   & da árvore de solução e escolhida para continuar a construção\\
%   $reqEscolhida$ & requisição escolhida para continuar a construção da árvore\\
%   $servRaiz$ & 1, para o servidor raiz da árvore de propagação das variáveis duais\\
%   $numCiclo$ & número de ciclos descobertos em um passo\\
%   $idCicloServ$ & id do ciclo que o servidor pertence\\
%   $cicloServ$ & caminho do ciclo na qual o servidor pertence  \\
%   $cicloServTam$ & tamanho do ciclo na qual o servidor pertence  \\
%   $posCicloServ$ & posição que o servidor está no ciclo que ele pertence\\ 
%   $crServ$ & custo reduzido do ciclo que o servidor pertence\\
%   $funcServ(c_{p})$ & função que retorna o servidor da posição $p$ do caminho (ciclo) $c$\\     
%   $teta$ & valor do $\theta$ do ciclo que o servidor pertence\\
%   $recAtualizaU_{s}$ & 1, se o servidor recebeu atualização da variável dual u referente ao\\
%   &ciclo de $s$ e 0, caso contrário\\
%   $dualV_{r}$ & valor da variável dual $v$ associado à requisição $r$\\
%   $servPaiDV_{r}$ & servidor pai da variável dual $v$ associado à requisição $r$\\
%   $participa_{rs}$ & 1, se a atribuição da requisição $r$ ao servidor $s$ pertence a solução,\\
%   & e 0, caso contrário\\
%   $caminhoReq^{r}$ & caminho na árvore de solução $T$ da raiz $sT$ até a requisição $r$\\
%   $caminhoReqTam_{r}$ & tamanho do caminho na árvore de solução $T$ da raiz $sT$ até a\\
%   &requisição $r$\\
%   $c_{i}$ & posição $i$ do caminho $c$\\
%   $idCicloReq_{r}$ & id do Ciclo que a requisição $r$ pertence\\
%   $cicloReq_{r}$ & caminho do ciclo na qual a requisição $r$ pertence\\
%   $cicloReqTam_{r}$ & tamanho do ciclo na qual a requisição $r$ pertence\\
%   $posCicloReq_{r}$ & posição que a requisição $r$ está no ciclo que ela pertence\\
%   $crReq_{r}$ & custo reduzido do ciclo que a requisição $r$ pertence\\
%   $funcReq(c_{p})$ & função que retorna a requisição da posição $p$ do caminho $c$, (se a\\
%   &posição corresponder a de um servidor,  o valor $-1$ é retornado)\\ 
%   $funcCont(c_{p})$ & função que retorna o conteúdo da requisição da posição $p$ do ca- \\
%   &minho ou ciclo $c$ (se a posição corresponder a de um servidor, o\\
%   &valor $-1$ é retornado)\\
%   $tetaReq_{r}$ & valor do $\theta$ do ciclo que requisição $r$ pertence\\
%   $recAtualizaUReq_{rs}$ & 1, se a requisição $r$ recebeu atualização da variável dual $u$  refe-\\
%   &rente ao ciclo de $s$ e 0, caso contrário\\
%   $servAtingidos$ & conjunto dos servidores atingidos pelas mensagens de cálculo \\
%   &das variáveis duais da construção da árvore de solução\\
%   $servCicloIniciado$ & conjunto dos servidores que iniciaram o processo de descoberta \\ 
%   &de ciclo\\
%   $varSainte$ & conjunto relacionado a variável que sai da solução, $\{req,$ \\
%   & $ servReq, serv,$   $paiReq, ciclo, r, pos\}$ em que $req$ é a requisição \\
%   & relacionada à atribuição que sai da solução, $servReq$ é o servi-\\
%   & dor na qual $req$ pertence, $serv$ é o servidor relacionado\\
%   & à atribuição que sai da solução, $paiServ$ é o nó pai de \\ 
%   & $reqT(req,serv)$ na árvore $T$, $ciclo$ é o id do ciclo que originou\\
%   & a saída da variável, $r$ é a requisição responsável por $ciclo$ e\\
%   & $pos$ é a posição de $req$ no $ciclo$\\
%   $servVaru$ & lista dos servidores que enviaram o valor da variável dual $u$\\
%   $varu_s$ & conjunto de valores duais $u$ dos servidores, onde $varu_s$ é o valor $u$ de $s$\\   
%   \end{tabular}

